Capacitively-coupled resonators for terahertz planar-Goubau-line filters

Low-loss planar Goubau lines show promising potential for terahertz applications. However, a single-wire waveguide exhibits less design freedom than standard multi-conductor lines, which is a significant constraint for realizing standard components. Existing filters for planar Goubau line lack clear design procedures preventing the synthesis of an arbitrary filter response. In this work, we present a design for a bandpass/bandstop filter for planar Goubau line by periodically loading the line with capacitively coupled {\lambda}/2 resonators, which can be easily tuned by changing their electrical length. The filter's working principle is explained by a proposed transmission-line model. We designed and fabricated a passband filter centered at 0.9 THz on a 10-{\mu}m silicon-membrane substrate and compared measurement results between 0.5 THz and 1.1 THz to electromagnetic simulations, showing excellent agreement in both S11 and S21. The measured passband has an insertion loss of 7 dB and a 3-dB bandwidth of 31 %. Overall, the proposed filter design has good performance while having a simple design procedure.

==> MySettings.tex <==
\usepackage{amsfonts} 
\usepackage{color}
\usepackage[version=4]{mhchem}
\usepackage{pgfplots}
\usepackage{siunitx}
\usepackage{circuitikz} % For drawing circuits
    \usetikzlibrary{decorations.markings}
    \usepackage{adjustbox}
    \usepackage{adjustbox}
\usepackage{hyperref}
\usepackage{stix}
\usepackage{tikz}
\RequirePackage{tikz} % For Orcid icon

%% ORCID
% Make Orcid icon
\definecolor{lime}{HTML}{A6CE39}
\newcommand{\orcidicon}{%
	\begin{tikzpicture}
	\draw[lime, fill=lime] (0,0) 
		circle [radius=0.16] 
		node[white] {{\fontfamily{qag}\selectfont \tiny ID}};
	\draw[white, fill=white] (-0.0625,0.095) 
		circle [radius=0.007];
	\end{tikzpicture}
	\hspace{-2mm}
}
% Define link and button for each author
\foreach \x in {A, ..., Z}{%
\expandafter\xdef\csname orcid\x\endcsname{\noexpand\href{https://orcid.org/\csname orcidauthor\x\endcsname}{\noexpand\orcidicon}}
}

\usepackage{amsmath}% for double integral symbol in this template
\usepackage{graphicx}% for figures
\usepackage{multirow}% to allow multiple-row elements in tabular environment
\usepackage[none]{hyphenat}% turn off hyphenation to make text extraction and indexing easier
\usepackage{float}% better control of floating figures and tables
\usepackage{subfig}% for subfigures within figures
\captionsetup{font=footnotesize}
\usepackage{dblfloatfix}% fix to allow page-wide floats at bottom of page
\usepackage{siunitx}
\newcommand{\SIadj}[2]{\SI[number-unit-product={\text{-}}]{#1}{#2}}

\usepackage{hyperref}
\usepackage{amsfonts} 

\usepackage{tabularx}
\usepackage{booktabs}

==> Settings.tex <==
% BASIC SETTINGS
\usepackage{caption}
\usepackage{commath}
\usepackage{graphicx, epstopdf}                                                           % Figures
\usepackage{longtable}
\usepackage{mwe}
\setlength{\parskip}{0em}
\usepackage{subcaption}

\usepackage{moreverb}                                                           % List settings
\usepackage{textcomp}                                                           % Fonts, symbols etc.
\usepackage{lmodern}                                                            % Latin modern font
\usepackage{helvet}                                                             % Enables font switching
\usepackage[T1]{fontenc}                                                        % Output settings
%\usepackage[swedish]{babel}                                                    % Language settings
\usepackage[utf8]{inputenc}                                                     % Input settings
\usepackage{amsmath}                                                            % Mathematical expressions (American mathematical society)
\usepackage{amssymb}                                                            % Mathematical symbols (American mathematical society)
\usepackage{subfig}                                                                     % Enables subfigures
\usepackage{listings}                                                           % Enables source code listings
\usepackage{chemfig}                                                    % Chemical structures
\usepackage{siunitx}
\usepackage[a4paper, total={15cm, 23.7cm}]{geometry}
%\usepackage[top=3cm, bottom=3cm,inner=3cm, outer=3cm]{geometry}                 % Page margin lengths                  
\usepackage{eso-pic}                                                            % Create cover page background
\newcommand{\backgroundpic}[3]{
        \put(#1,#2){
        \parbox[b][\paperheight]{\paperwidth}{
        \centering
        \includegraphics[width=0.8\paperwidth,height=\paperheight,keepaspectratio]{#3}}}}
       
        
\usepackage{csquotes}
\usepackage{filecontents} 

%

% OPTIONAL SETTINGS (DELETE OR COMMENT TO SUPRESS)
%\usepackage{color}
\usepackage{comment}
\usepackage{lipsum}
\usepackage{float}
\usepackage{hyperref}
\usepackage{pgfgantt}
\usepackage{etoolbox}
\usepackage{placeins}
\usepackage{xpatch}
\usepackage{siunitx}
\usepackage[super]{nth}
\usepackage{titlesec}
\usepackage{pdfpages}
\usepackage[numbers]{natbib}
\usepackage{units}

%% MATLAB-code fix

\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}

\lstset{ %
  backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}
  basicstyle=\footnotesize,        % the size of the fonts that are used for the code
  breakatwhitespace=false,         % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  captionpos=b,                    % sets the caption-position to bottom
  commentstyle=\color{mygreen},    % comment style
  deletekeywords={...},            % if you want to delete keywords from the given language
  escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  frame=single,                    % adds a frame around the code
  keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
  keywordstyle=\color{blue},       % keyword style
  language=Matlab,                 % the language of the code
  morekeywords={*,...},            % if you want to add more keywords to the set
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\tiny\color{mygray}, % the style that is used for the line-numbersf
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=2,                    % the step between two line-numbers. If it's 1, each line will be numbered
  stringstyle=\color{mymauve},     % string literal style
  tabsize=2,                       % sets default tabsize to 2 spaces
  title=\lstname                   % show the filename of files included with \lstinputlisting; also try caption instead of title
}


\epstopdfsetup{outdir=./}
\graphicspath{{./fig/}}

==> include/Papers_to_cite.tex <==
\section{Papers to cite}

\begin{itemize} 
    \item "Terahertz Microfluidic Metamaterial Biosensor for Tiny Volume Liquid Samples" \cite{Zhang2019a}
\end{itemize}


==> old/old_fabsteps.tex <==

    \begin{enumerate}
        \item  Initial 20~mm by 20~mm  silicon-on-insulator wafer purchased from University Wafers. Top layer: $\SI{10}{\um}$ thick high-resistivity (>$\SI{10}{k\ohm.cm}$ float-zone) silicon. Oxide layer: $\SI{1}{\um}$ thick SiO$_2$.
        Bulk: $\SI{400}{\um}$ thick silicon.
        \item Spin of the electron-beam lithography resist and auxiliary layers:
        HMDS process \SI{100}{\celsius} 60 seconds.
        Spin MMA 8.5 EL10 (\SI{450}{\nm} thick) at \SI{3000}{rpm} for \SI{30}{\second}. Acceleration time: \SI{1}{\second}. Bake at \SI{110}{\celsius} for \SI{10}{\min}.
            Spin PMMA A2 (\SI{70}{\nm} thick) at \SI{3000}{rpm} for \SI{30}{\second}. Acceleration time: \SI{1}{\second}. Bake at \SI{110}{\celsius} for \SI{10}{\minute}.
        %
        \item e-beam lithography (current \SI{120}{\nA}, initial dose \SI{320}{\micro\coulomb /\cm^2}).
        %
        \item Substrate development: Developed in IPA:DI-H$_2$O in 10:1 volume ratio for 40 seconds. Ash O$_2$ plasma at \SI{40}{\watt} for \SI{5}{\second}.
        
        \item Deposited Ti/Au 100/3500 \si{\angstrom}.
        
        \item Lift-off in \SI{65}{\celsius} acetone and \SI{65}{\celsius} IPA.
        %
        \item Turn chip face down. Sputtering $\SI{20}{nm}$ of aluminum on backside of SOI chip. HMDS process at \SI{100}{\celsius} for 60 seconds. Spin SPR220-3.0  at \SI{3000}{rpm} for \SI{30}{\second}. Acceleration time: \SI{0.3}{\second}. Bake on hot-plate for \SI{90}{\second} at \SI{115}{\celsius}. Laser writer exposure.
        
        \item Develop resist and continue etching aluminum in MF24A.
        
        \item  Spin resist AZ4562 on 6-inch carrier wafer at \SI{3000}{rpm} for \SI{30}{\second}. Acceleration time: \SI{0.3}{\second}. No baking. Place SOI chip face down and gently press it into the carrier wafer. Bake at \SI{120}{\celsius} for \SI{90}{\minute}.
        Deep reactive-ion etching (Bosch process). Gases: $\text{SF}_6+\text{O}_2$. Passivation: C$_2$F$_8$. Etching rate: $\SI{1}{\um}$ per cycle.
        
        \item After etching, leave 48 hours in room temperature acetone to detach chip from carrier wafer by dissolving the resist AZ4562.
        
        \item Remove resist residues with O$_2$ plasma.
        
    \end{enumerate}
